ARCH: Efficient Adversarial Regularized Training with Caching

Adversarial regularization can improve model generalization in many natural language processing tasks. However, conventional approaches are computationally expensive since they need to generate a perturbation for each sample in each epoch. We propose a new adversarial regularization method ARCH (adversarial regularization with caching), where perturbations are generated and cached once every several epochs. As caching all the perturbations imposes memory usage concerns, we adopt a K-nearest neighbors-based strategy to tackle this issue. The strategy only requires caching a small amount of perturbations, without introducing additional training time. We evaluate our proposed method on a set of neural machine translation and natural language understanding tasks. We observe that ARCH significantly eases the computational burden (saves up to 70% of computational time in comparison with conventional approaches). More surprisingly, by reducing the variance of stochastic gradients, ARCH produces a notably better (in most of the tasks) or comparable model generalization. Our code is available at https://github.com/SimiaoZuo/Caching-Adv.

==> 0-broader-impact.tex <==
\section*{Broader Impact}
\vspace{-0.05in}

This paper proposes a caching method to speedup adversarial regularized training for NLP tasks.
Our proposed method provides a fundamental way to address the efficiency issue that commonly exists in conventional adversarial regularization methods.
We use publicly available data, to conduct neural machine translation and natural language understanding experiments. Our framework is built using public code bases.
We do not find any ethical concerns.
